Tunable layered-magnetism-assisted magneto-Raman effect in a two-dimensional magnet $\mathrm{CrI_3}$

We use a combination of polarized Raman spectroscopy experiment and model magnetism-phonon coupling calculations to study the rich magneto-Raman effect in the two-dimensional (2D) magnet $\mathrm{CrI_3}$. We reveal a novel layered-magnetism-assisted phonon scattering mechanism below the magnetic onset temperature, whose Raman excitation breaks time-reversal symmetry, has an antisymmetric Raman tensor, and follows the magnetic phase transitions across critical magnetic fields, on top of the presence of the conventional phonon scattering with symmetric Raman tensors in $N$-layer $\mathrm{CrI_3}$. We resolve in data and by calculations that the 1st-order $A_g$ phonon of monolayer splits into a $N$-fold multiplet in $N$-layer $\mathrm{CrI_3}$ due to the interlayer coupling ($N$>=2) and that the phonons with the multiple show distinct magnetic field dependence because of their different layered-magnetism-phonon coupling. We further find that such a layered-magnetism-phonon coupled Raman scattering mechanism extends beyond 1st-order to higher-order multi-phonon scattering processes. Our results on magneto-Raman effect of the 1st-order phonons in the multiplet and the higher-order multi-phonons in $N$-layer $\mathrm{CrI_3}$ demonstrate the rich and strong behavior of emergent magneto-optical effects in 2D magnets and underlines the unique opportunities of new spin-phonon physics in van der Waals layered magnets.

==> LaTeX 1/author_list.tex <==
% Author list

\author{Wencan Jin}
\altaffiliation{current affiliation: Department of Physics, Auburn University, 380 Duncan Drive, Auburn, AL 36849, USA}
\affiliation{Department of Physics, University of Michigan, 450 Church Street, Ann Arbor, Michigan 48109, USA}


\author{Zhipeng Ye}
\affiliation{Department of Electrical and Computer Engineering, 910 Boston Avenue, Texas Tech University, Lubbock, Texas 79409, USA}

\author{Xiangpeng Luo}
\affiliation{Department of Physics, University of Michigan, 450 Church Street, Ann Arbor, Michigan 48109, USA}

\author{Bowen Yang}
\affiliation{Institute for Quantum Computing, Department of Chemistry, and Department of Physics and Astronomy, University of Waterloo, Waterloo, 200 University Ave W, Ontario N2L 3G1, Canada}

\author{Gaihua Ye}
\affiliation{Department of Electrical and Computer Engineering, 910 Boston Avenue, Texas Tech University, Lubbock, Texas 79409, USA}

\author{Fangzhou Yin}
\affiliation{Institute for Quantum Computing, Department of Chemistry, and Department of Physics and Astronomy, University of Waterloo, Waterloo, 200 University Ave W, Ontario N2L 3G1, Canada}

\author{Hyun Ho Kim}
\altaffiliation{current affiliation: School of Materials Science and Engineering, Kumoh National Institute of Technology, Gumi, Gyeongbuk 39177, Korea}
\affiliation{Institute for Quantum Computing, Department of Chemistry, and Department of Physics and Astronomy, University of Waterloo, Waterloo, 200 University Ave W, Ontario N2L 3G1, Canada}

\author{Laura Rojas}
\affiliation{Department of Electrical and Computer Engineering, 910 Boston Avenue, Texas Tech University, Lubbock, Texas 79409, USA}

\author{Shangjie Tian}
\affiliation{Department of Physics and Beijing Key Laboratory of Opto-electronic Functional Materials \& Micro-nano Devices, Renmin University of China, Beijing 100872 China}

\author{Yang Fu}
\affiliation{Department of Physics and Beijing Key Laboratory of Opto-electronic Functional Materials \& Micro-nano Devices, Renmin University of China, Beijing 100872 China}

\author{Shaohua Yan}
\affiliation{Department of Physics and Beijing Key Laboratory of Opto-electronic Functional Materials \& Micro-nano Devices, Renmin University of China, Beijing 100872 China}

\author{Hechang Lei}
\affiliation{Department of Physics and Beijing Key Laboratory of Opto-electronic Functional Materials \& Micro-nano Devices, Renmin University of China, Beijing 100872 China}

\author{Kai Sun}
\affiliation{Department of Physics, University of Michigan, 450 Church Street, Ann Arbor, Michigan 48109, USA}

\author{Adam W. Tsen}
\affiliation{Institute for Quantum Computing, Department of Chemistry, and Department of Physics and Astronomy, University of Waterloo, Waterloo, 200 University Ave W, Ontario N2L 3G1, Canada}

\author{Rui He}
\email{rui.he@ttu.edu}
\affiliation{Department of Electrical and Computer Engineering, 910 Boston Avenue, Texas Tech University, Lubbock, Texas 79409, USA}

\author{Liuyan Zhao} 
\email{lyzhao@umich.edu}
\affiliation{Department of Physics, University of Michigan, 450 Church Street, Ann Arbor, Michigan 48109, USA}


